Representable bimodules over C*-algebras

Given two C*-algebras A and B, abstract A-B bimodules that can be isometrically represented as operator bimodules are characterised in terms of their norm. Various properties of such bimodules are given. Their theory is very similar to those of classical normed spaces.

==> final_sec1.tex <==
%auto-ignore
\nobreak
\begin{section}{Introduction}

Soient $A$, $B$ deux $C^*$-alg\`ebres. On consid\`ere dans la suite
des $A-B$ bimodules norm\'es $V$ tels que les actions de $A$ et $B$ sont
continues et essentielles, c'est \`a dire que
\begin{equation*}
  \label{def_bimodule}
  \overline{AV}=\overline{VB}=V.
\end{equation*}
Evidemment, si $A$ poss\`ede une unit\'e, alors $1v=v$, pour
tout $v\in V$ et cela est valable aussi pour l'action \`a droite de
$B$.

Dans \cite{ces} et \cite{er1} on donne une caract\'erization
abstraite des $A$--$B$ bimodules $V$, ayant une structure d'espace
d'op\'erateurs telle qu'il existe un espace de Hilbert
$\mf{H}$, deux repr\'esentations $\pi:A\to\mathcal{B}
(\mf{H})$, $\rho:B\to\mathcal{B} (\mf{H})$ et une
application \emph{compl\`etement isom\'etrique}
$J:V\to\mathcal{B}(\mf{H})$ v\'erifiant
\begin{equation*}
  J(avb)=\pi(a)J(v)\rho(b),\quad\forall a\in A,b\in B,v\in V.
\end{equation*}
Un tel $A-B$ bimodule est appel\'e dans~\cite{er1} \emph{$A-B$ bimodule
d'o\-p\'e\-ra\-teurs}. Nous on va l'appeller $A-B$ bimodule $L^\infty$ 
matriciellement norm\'e. Evidemment un tel espace est un $A-B$ bimodule 
norm\'e, o\`u les actions de $A$ et $B$ sont d\'efinies par
\begin{equation*}
  a.v.b=\pi(a)v\pi(b).
\end{equation*}
En outre, pour tout $a_1,a_2\in A$, $b_1,b_2\in B$ et $v_1,v_2\in V$ on a
\begin{equation*}
  \|a_1v_1b_1+a_2v_2b_2\|\le\|a_1a_1^*+a_2a_2^*\|^{1/2}
  \|b_1^*b_1+b_2^*b_2\|^{1/2}\max\{\|v_1\|,\|v_2\|\},
\end{equation*}
condition qu'on va appeller condition $(R)$.

Dans la suite on va d\'emontrer la r\'eciproque. Plus pr\'ecis\'ement,
on d\'emontre que un $A-B$ bimodule satisfait la condition $(R)$
si et seulement si il existe un espace de Hilbert $H$, deux
repr\'esentations $\pi$, $\rho$ de $A$ et $B$ dans
$\mathcal{B}(H)$ et un morphisme \emph{isom\'etrique} de $A-B$
bimodules $j:V\to\mathcal{B}(H)$ tel que
\begin{equation*}
  j(avb)=\pi(a)j(v)\rho(b),\quad\forall a\in A,b\in B,v\in V.
\end{equation*}
On va appeller des tels bimodules \emph{$A-B$ bimodules repr\'esentables}
($R$ comme $R$uan ou $R$epr\'esentables).
Le cas $A=B=\mathbb{M}_n$ a \'et\'e d\'ej\`a trait\'e dans
\cite[th\'eor\`eme I.1.9]{leh1}. Le cas commutatif $A=B=C_0(X)$ o\`u
les actions \`a droite et \`a gauche co\"\i ncident a \'et\'e
trait\'e dans \cite{hof}.
\end{section}  

Dans la section 2 on demontre quelque r\'esultats techniques utiles pour la
suite. L'ingr\'edient principal est le lemme fondamental~\ref{pici}, qui 
sert \`a
caract\'eriser les formes lin\'eaires born\'es sur les $A-B$ bimodules
repr\'esentables. 

Pour une repr\'esentation $(\pi,\mf{H})$ d'une $C^*$-alg\`ebre $C$ on
introduit la notion de \emph{localement cyclicit\'e}.
\begin{deffs}
  Soit $C$ est une $C^*$-alg\`ebre. Une repr\'esentation $(\pi,H)$ de
  $C$ est appel\'ee \emph{localement cyclique} si il existe 
  $\mathcal{E}\subset H$ un sous-ensemble dense dans $H$ tel que pour tout
  $h_1,h_2,\ldots,h_n\in\mathcal{E}$ il existe $h\in\mathcal{E}$ tel que 
  $h_i\in\overline{\pi(C)h}$.
\end{deffs}

Cette propri\'et\'e a \'et\'e remarqu\'e dans~\cite{sm1}, o\`u on consid\`ere
$A,B\subset\mathcal{B}(\mf{H})$ deux $C^*$ alg\`ebres et $V\subset\BH$ un
$A-B$ bimodule. Alors si $A\hookrightarrow\BH$ et $B\hookrightarrow\BH$ sont
localement cycliques, pour tout morphisme de $A-B$ bimodules $R:V\to\BH$
on a
\begin{equation*}
  \|R\|=\|R\|_{cb}.
\end{equation*}
Alors on peut d\'eduire, \`a partir des r\'esultats de~\cite{sue} (qui
font appel au th\'eor\`eme de Wittstock), le r\'esultat de prolongement
suivant: supposons $V\subset W\subset\BH$ sont deux $A-B$ bimodules
(essentiels) et $R:V\to\BH$ est un morphisme born\'e de $A-B$ bimodules.
Alors si $A\hookrightarrow\BH$ et $B\hookrightarrow\BH$ sont localement 
cycliques, il
existe un morphisme de $A-B$ bimodules $\tilde{R}:W\to\BH$ qui prolonge $R$,
tel que $\|\tilde{R}\|=\|R\|$.

Dans la section 2 on donne une d\'emonstration directe de cette derni\`ere
assertion, sans utiliser le th\'eor\`eme de Wittstock. Par ailleurs, 
le th\'eor\`eme de Wittstock est une cons\'equence du th\'eor\`eme de
prolongement, grace \`a la propri\'et\'e remarquable de l'alg\`ebre des
op\'erateurs compacts $\mathcal{K}$ de $l^2$, notamment que toutes les
repr\'esentations de $\mathcal{K}$ sont localement cycliques.

Dans la section 3 on introduit les repr\'esentations de $A-B$ bimodules 
norm\'es et on caract\'erise les bimodules repr\'esentables. On introduit les
espaces duaux de $A-B$ bimodules, g\'en\'eralisant le cas classique des espaces
norm\'es. 

Dans la section 4 on demontre que, \'etant donn\'e un $A-B$ bimodule norm\'e,
il existe sur $V$ une structure $L^\infty$ matricielle compatible si et 
seulement si $V$ est repr\'esentable. Parmi toutes les structures $L^\infty$
matricielles compatibles il existe une qui est minimale, et qu'on 
caract\'erise. Plus pr\'ecis\'ement, on a
\begin{thms}
  Soit $(V,(\|\cdot\|_n)_n)$ un $A-B$ bimodule $L^\infty$
  matriciellement norm\'e.
  Les affirmations suivantes sont equivalentes:
  \begin{enumerate}
  \item[(a)] La structure matricielle de $V$ est minimale.
  \item[(b)] Il existe $\Omega$ un compact et un morphisme de $A-B$
    bimodules compl\`etement isom\'etrique $V\to
    C(\Omega,\mathcal{B}(\kk{B''}, \kk{A''}))$.
  \item[(c)] Tout morphisme isom\'etrique $j:V\to
    C(\Omega,\mathcal{B}(\kk{B''},\kk{A''}))$ est compl\`etement
    isom\'etrique.
  \item[(d)] Pour $[v_{kl}]\in\mathbb{M}_n(V)$ on a
    \begin{equation*}
    \|[v_{kl}]\|_n=\sup\{\|\sum_{k=1}^n\sum_{l=1}^na_kv_{kl}b_l\|\ :
    \ \|\sum_{k=1}^na_ka_k^*\|\le1,\|\sum_{l=1}^nb_l^*b_l\|\le1\}.      
    \end{equation*}
  \item[(e)] Pour tout $A-B$ bimodule $L^\infty$ matriciellement norm\'e, 
    tout morphisme contractif de $A-B$ bimodules $W\to V$ est
    compl\`etement contractif.
  \end{enumerate}
\end{thms}
Comme cons\'equence directe on donne une autre d\'emonstration du 
th\'eor\`eme de repr\'esentation de~\cite{er1}.

Finalement, dans la section 5 on reprend les m\^emes questions, en ajoutant
des hypoth\`eses de dualit\'e. On d\'efinit las $A-B$ bimodules 
repr\'esentables duaux (qui sont tels qu'en enllevant la propri\'et\'e $(R)$
on retrouve la d\'efinition de~\cite{kr1}). On caract\'erise ces objets,
avec ou sans hypoth\`eses de normalit\'e pour les actions de $A$ et $B$.

Ces r\'esultats seront utiles pour l'\'etude des produits tensoriels 
relatifs des bimodules repr\'esentables, actuellement en cours.

